State Frequency Estimation for Anomaly Detection

Many works have studied the efficacy of state machines for detecting anomalies within NetFlows. These works typically learn a model from unlabeled data and compute anomaly scores for arbitrary traces based on their likelihood of occurrence or how well they fit within the model. However, these methods do not dynamically adapt their scores based on the traces seen at test time. This becomes a problem when an adversary produces seemingly common traces in their attack, causing the model to miss the detection by assigning low anomaly scores. We propose SEQUENT, a new unsupervised approach that uses the state visit frequency of a state machine to adapt its scoring dynamically for anomaly detection. SEQUENT subsequently uses the scores to generate root causes for anomalies. These allow the grouping of alarms and simplify the analysis of anomalies. We evaluate SEQUENT's effectiveness in detecting network anomalies on three publicly available NetFlow datasets and compare its performance against various existing unsupervised anomaly detection methods. Our evaluation shows promising results for using the state visit frequency of a state machine to detect network anomalies.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sec_encoding_algorithm.tex <==
\section{Encoding Algorithm}\label{sec:encoding_algorithm}
In this section, we describe our encoding algorithm for NetFlow data. We first explain how we compute the context for each unique flow feature value and how we use the context to create its encoding. Then we provide implementation details of our encoding algorithm. Our encoding algorithm is publicly available at~\cite{encode_repo}

%\subsection{Goal of Algorithm}
%The goal of our algorithm is to learn an encoding for a given set of NetFlow features that captures the different network behaviours in the network. We do so by using the frequency of the feature values to compute a context in which the values occur. We assume that by being able to compute a context in which a feature value occurs, we can use the context to group similar network behaviours together. Having this group of network behaviours that can occur in the network, we can learn behavioural information that is not trivially seen in the NetFlow data and therefore also not learned by the models.

\subsection{Computing the Context}
Our idea to compute the context for the values of a given NetFlow feature is inspired by the work of Word2Vec, especially the Count Bag of Words (CBOW) method~\cite{Mikolov2013_efficient}. For each value $v$ of a given non-categorical NetFlow feature $f$, we want to compute the context in which $v$ occurs. This is done by computing the frequencies of the values that occurred directly before $v$ and the frequency of the values that occurred directly after $v$. The intuition is that the frequencies of the previous/next values capture the behaviour of $v$ within the network i.e. which other feature values does $v$ co-occur with and how often.

The computed frequencies are used to generate a vector for value $v$. Before the context frequencies are computed for each value $v$, the NetFlow data is first grouped based on the connection (i.e. grouped by the pair of source and destination host). This ensures the context of $v$ is not influenced by other flows co-occurring in the same network. The context thus represents the surrounding flows generated by the same (kind of) software.
%We assume a software creates one is to make sure that we only compute frequencies for the direct previous/next values that have occurred within the same connection that $v$ has occurred in. 
%Without this constraint, values that occurred in different connections (and thus also have a different meaning) will incorrectly be used for computing the context of $v$. 

%Since the Euclidean distance is computed using pair-wise difference between the elements in the vector, the indices in the vector are very import for our similarity definition between the vectors i.e. the frequency of the direct previous/next values each $v$ must be stored at the exact same index in the vector. If the locations of the frequencies differ between two vectors, then this results in a large distance between the vectors. As an example, say we have two similar values $v_1 = [1, 2,0,0]$ and $v_2 = [1, 1,0,0]$, where the first two elements of the vector are used to store the frequencies of direct previous values and the last two elements are used to store the frequencies of the direct next values. If we compute the Euclidean distance between $v_1$ and $v_2$, then we get $v1 - v2 = 1$ as result. But if now we switch the positions around for how we store the frequency values, such that $v_2 = [0,0, 1, 2]$, then the new Euclidean distance between these two values will result to $v_1 - v_2 = 3.87$. This is much larger than what we had before then the positions of the frequency values are fixed for all vectors. Therefore, the positions in the vectors are important for defining similarity between feature values in this work. 

\subsection{Creating the Encoding}
From the context generation, we obtain vectors containing frequencies. We use Euclidean distance to discover whether two feature values $v$ and $v'$ occur in similar contexts. The smaller the distance between two vectors, the more similar the context in which two feature values occur. This provides us with the ability to create groups of contextually similar feature values.

%As use the distances of the vectors to define the context of each unique feature value $v$, we can use these vectors to group similar (unique) feature values together.
The encoding for the feature values are are created by clustering the vectors of the feature values and the assigned cluster labels are used as the encoding for the feature values. Thus, the encoding for $v$ is the corresponding cluster label that was assigned to its vector. Similar feature values that have similar frequency values and occur in a similar context would therefore be assigned to the same cluster and would get the same encoding. For the clustering of the vectors, we have chosen the KMeans algorithm as this algorithm gives us control over the number of clusters that can be formed i.e. giving us control over the size of the encoding for each non-categorical feature on which we want to compute the encoding. Though we have chosen to use KMeans as our clustering algorithm, it is also possible to use any other clustering algorithm to compute the encoding.

\subsection{An Illustrative Example}
We now provide a small illustrative example of how our encoding is computed for NetFlow data. The data that is used in this example is a very small subset of NetFlow data extracted from one of the datasets (UGR-16 dataset) that is used in our evaluation. Figure~\ref{fig:ugr_small_netflow_sample} presents the small subset of data that we will in our example. More information on this dataset is given in Section~\ref{sect-evaluation}. In this example, we show how we compute the context and the encoding for the unique byte values. 

First, we find the unique byte values. From the byte values that are shown in Figure~\ref{fig:ugr_small_netflow_sample}, we see a total of nine unique byte values: 64, 165, 977, 1224, 1540, 2852, 2909, 3149 and 3169. Note that all data in this example comes from the same connection. Then we compute the frequencies of the direct previous/next byte values for each of these nine byte values. The computed frequencies are shown in Figure~\ref{fig:ugr_small_example_frequency}. Each row that is shown in Figure~\ref{fig:ugr_small_example_frequency} is used as the vector for the corresponding unique byte value. The vectors are then clustered together using the KMeans algorithm and the assigned cluster labels for the vectors are used as the encoding for the corresponding unique byte values. Figure~\ref{fig:ugr_small_example_encoding} presents the assigned cluster labels for each unique byte value.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figures/ugr_16_small_sample.pdf}
    \caption{A very small subset of NetFlow data extracted from the UGR-16 dataset. This small subset is extracted to be used for the illustrative example of our encoding.}
    \label{fig:ugr_small_netflow_sample}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/ugr_16_small_sample_frequencies}
    \caption{ Frequencies of the direct previous/next bytes values for each of the unique byte values that are present in Figure~\ref{fig:ugr_small_netflow_sample}.}
    \label{fig:ugr_small_example_frequency}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{figures/ugr_16_small_sample_encoding.pdf}
    \caption{Cluster labels assigned to the unique byte values used in the example. The assigned cluster labels are used as the encoding for the unique byte values. In this example, we have used five clusters to cluster the vectors.}
    \label{fig:ugr_small_example_encoding}
\end{figure}


\subsection{Implementation Details}
As shown in our illustrative example, a vector is generated for each unique feature value $v$. As these vectors are clustered together using KMeans, the sizes of the vectors must have the same size. Furthermore, all vectors must store the same information (frequency values regarding a particular feature value) at the exact same position. % as this is very important for defining similarity between feature values within this work. 
%Due to these two properties that must hold for each vector that we generate, we must therefore have a generalised structure for all vectors.

As shown in Figure~\ref{fig:ugr_small_example_frequency}, the first half of each vector (marked in brown) stores the frequencies of the direct previous values and the second half (marked in blue) stores the frequencies of the direct next values. Furthermore, the size of each vector is equal to twice the number of unique feature values. This is to make sure that each vector has the same structure and size. The structure in Figure~\ref{fig:ugr_small_example_frequency} is a step in the right direction, but it does have limitations: 

\begin{itemize}
    \item It could create many sparse vectors. 
    \item The size of each feature depends on the number of unique values for a given feature. If the number grows very large, then the size of the vectors would also grow very large.
    %This removes the control that we can have on the size of the vectors.
    \item We cannot capture the behaviour in which a feature value $v$ occurs frequently with itself. We frequently observe in NetFlow data that the previous/next value of $v$ is itself, indicating repetitive software behaviour.
\end{itemize} 

This last limitation is somewhat tricky. The counts of the value itself are somewhere in the table. For instance, for value 64 in Table~\ref{fig:ugr_small_example_frequency} it is in the column labeled 64. The issue is that for different data rows, these self-contexts are in different columns. Thus rows with only self-contexts would receive a large distance. In our view, such repetitive behaviour is indicative of similar software and should not depend on the exact flow value. 

We resolve this we add two columns to store the previous self-frequency and the next self-frequency. The self-frequency refers to the frequency in which $v$ has itself as its previous/next value. In addition to storing the self-frequency, we have also included an additional entry that stores the logarithm of the frequency of $v$ (marked in red). This way the frequency of $v$ also influences the distance computation between vectors. Furthermore, this entry helps to differentiate features that have similar previous/next values but different frequencies.

%As we are clustering the vectors to create the encoding, the length of the vectors must be equal for all feature values. As each feature value $v$ would have a different set of previous/next values, we need to have a generalised structure for the vector. During the implementation of our encoding algorithm, we have experimented with different methods in how to construct the vectors for each feature value $v$ of a given NetFlow feature $f$.

% For our first method, we used a method that is similar to Word2Vec; we used a vector to store the frequency of all possible previous/past values, including the frequency of $v$ itself. For the second method, we applied a time series differencing method to the values before computing the frequencies. The main issue with these two methods is that we are creating very large vectors to store the frequencies and we do not have control over the size of the vectors. 
% For our first method, a vector would have the length of two times the number of all possible feature values. The first half of the vector is used to store the frequencies of the previous values and the second half is used to store the frequencies of the next values. To capture behaviour in which a feature value $v$ occurs frequently with itself in the context (having a high-frequency value for itself in the previous/next values), we have introduced two extra entries in the vector that store the previous self-frequency and the next self-frequency respectively. This decision has led to the issue of having zeroes in the vectors at where the frequency values were supposed to be stored and the location of these entries would be different for each feature value $v$. As the distances between the vectors are used for clustering, these entries could lead to the incorrect grouping of feature values.

% The issue with the first method is that we have a very large vector for each feature value and we have introduced two zero entries in the vector that would cause incorrect grouping of feature values. To resolve these issues, we came up with a second method that computes the frequency of the absolute differences between feature value $v$ and its previous/next values. This method fixes the location in which we store the previous/next self-frequency; a difference of 0 means it is the same feature value and it is an occurrence with itself. Furthermore, using the differences would reduce the size of the vectors as we are looking at all possible absolute differences that can occur between feature values instead of all possible feature values.

% The second method resolves the issues that we had with the first method but the second method still suffers from the issue that we have a very large vector for each feature value as there can be many possible absolute differences between the feature values. 

To resolve the first two limitations, we divide the space of the previous and next values into ten bins each using percentiles. This gives a vector of length 20 for each feature value $v$. In fact, this solution gives us control over the size of the vector by changing the number of bins that are used to divide the space of the previous/next values.
%With this solution, instead of incrementing the frequencies of the exact previous/next values for $v$, we check which bin a previous/next value falls into and increment the frequency of the corresponding bin. 
Figure~\ref{fig:encoding_final_vector_structure} presents the final generalised structure that is used in the implementation of our encoding.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/encoding_generalised_vector_structure}
    \caption{Generalised vector structure that is used for each unique feature value within our encoding algorithm.}
    \label{fig:encoding_final_vector_structure}
\end{figure}


Since KMeans chooses the initial centroids at random, each run of KMeans could lead to different final clusters.  %This means that one run of KMeans does not guarantee the best clusters that can be formed for the given data. To resolve this issue, 
We therefore run KMeans ten times and take the best run to create our encoding for the unique feature values. We use the Silhouette Coefficient as our metric to evaluate how well the clusters were formed for the vectors that we have generated. To compute the Silhouette Coefficient, we use the python that is provided by scikit-learn~\cite{sklearn-silhouette}


Figure~\ref{fig:data_processing_pipeline} provides a high-level overview of our data processing pipeline. For the clustering of the vectors, we have used the KMeans Clustering implementation that is provided by Scikit-learn machine-learning package~\cite{sklearn_kmeans}. We opted to use KMeans clustering to cluster the vectors as we can fix the number of clusters that can be created and thus we can fix the size of our encoding. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/data_processing_pipeline}
    \caption{High-level overview of our data processing pipeline. The pipeline shows how the encoding is created for the given NetFlow input data using our encoding algorithm.}
    \label{fig:data_processing_pipeline}
\end{figure}

% \begin{algorithm}[!ht] 
% \caption{High-level overview of our encoding algorithm}
% \label{algo:encoding_algorithm}
% \begin{algorithmic}[1]
%     \State {$N$ $\gets$ netFlow\ data}
%     \State {$F$ $\gets$ selected\ features}
%     \State {$E$ $\gets$ empty\ mapping}
%     \For{$f$ in $F$}
%         \State {$V \gets$ feature values of $f$}
%         \State {$\lambda \gets$ empty list}
%         \For{$v$ in $V$}
%             \State {$\gamma \gets$ construct vector using the frequencies of previous/next values}
%             \State {$\lambda \gets \lambda \cup \gamma$}
%         \EndFor
%         \State {$E \gets E \cup KMeans(\lambda)$}
%     \EndFor
%     \State \Return {$E$}
% \end{algorithmic}
% \end{algorithm}
